Constrained nonlinear output regulation using model predictive control -- extended version

We present a model predictive control (MPC) framework to solve the constrained nonlinear output regulation problem. The main feature of the proposed framework is that the application does not require the solution to classical regulator (Francis-Byrnes-Isidori) equations or any other offline design procedure. In particular, the proposed formulation simply minimizes the predicted output error, possibly with some input regularization. Instead of using terminal cost/sets or a positive definite stage cost as is standard in MPC theory, we build on the theoretical results by Grimm et al. 2005 using a detectability notion. The proposed formulation is applicable if the constrained nonlinear regulation problem is (strictly) feasible, the plant is incrementally stabilizable and incrementally input-output to state stable (i-IOSS/detectable). We show that for minimum phase systems such a design ensures exponential stability of the regulator manifold. We also provide a design procedure in case of unstable zero dynamics using an incremental input regularization and a nonresonance condition. Inherent robustness properties for the noisy error/output-feedback case are established under simplifying assumptions (e.g. no state constraints). The theoretical results are illustrated with an example involving offset free tracking with noisy error feedback. The paper also contains novel results for MPC without terminal constraints with positive semidefinite input/output stage costs that are of independent interest.

==> OutputRegulation_MPC.tex <==
%!TEX root = ./OutputRegulation.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{MPC - semidefinite costs and set stabilization}
%\section{Model predictive control  \\ semidefinite costs and set stabilization}
\label{sec:MPC}
In this section, we study stability of nonlinear MPC schemes with positive semidefinite cost functions without any terminal ingredients (no terminal cost or terminal set), similar to~\cite{grimm2005model}. 
%The relevance of this problem to  output regulation and input-output models is discussed in Section~\ref{sec:output} and Remark~\ref{rk:IO_model}, respectively. 
 
\input{OutputRegulation_MPC_1}
\input{OutputRegulation_MPC_2}
\input{OutputRegulation_MPC_3}


 

\subsubsection*{Discussion}
\JK{der folgende satz ist doppelt (bereit nach Thm.~1 erwähnt, beim restructern aufpassen}
Note that Inequalities~\eqref{eq:Lyap_1}--\eqref{eq:Lyap_2} directly imply $\lim_{t\rightarrow\infty}\sigma(x_t)=0$. 
Furthermore, in case $\sigma(x)=\|x\|^a$, $a>0$, Theorem~\ref{thm:MPC}  ensures exponential stability of $x=0$.

In Section~\ref{sec:output}, as on of the main results of the paper, we show how the results in Theorem~\ref{thm:MPC} can be used to design an MPC scheme that implicitly solves the constrained output regulation problem. 
In the following, we briefly highlight the relevance of Thm.~\ref{thm:MPC} to the problem of MPC for input-output stage costs and models. 
% 
\begin{remark}
\label{rk:IO_model}
Similar to the considered problem of output regulation, input-output stage costs $\ell=\|y\|^2+\|u\|^2$ appear naturally in the case of trajectory tracking or path following, if only some output reference is specified as opposed to a full state reference~\cite{faulwasser2015nonlinear}. 
%Similarly
Likewise, in case an input-output model resulting from some system identification is used, e.g.  input-output LPV systems~\cite{abbas2018improved,cisneros2019stabilizing}, the consideration of positive semidefinite input-output stage costs is natural. 
 In all these results, a given state trajectory is considered and a suitable terminal cost (and terminal region) is constructed offline. Using Theorem~\ref{thm:MPC}, the need for constructing such terminal ingredients or determining the corresponding state trajectory can be dropped by choosing a  sufficiently  large $N$. 

The need to use a positive semidefinite input-output stage cost $\ell$ and avoid terminal ingredients or state references also appears in data-driven MPC, where (linear) models are implicitly represented using data~\cite{berberich2019data,coulson2019regularized}. 
However, offline verification of the corresponding \textit{detectability} and \textit{stabilizability} conditions (Ass.~\ref{ass:stab}, \ref{ass:detect}) with such an implicit data based model is still open research topic, compare e.g.~\cite{romer2019one} where some input-output system properties are verified for such data based models. 
\end{remark} 
